A lightweight and accurate YOLO-like network for small target detection in Aerial Imagery

Despite the breakthrough deep learning performances achieved for automatic object detection, small target detection is still a challenging problem, especially when looking at fast and accurate solutions suitable for mobile or edge applications. In this work we present YOLO-S, a simple, fast and efficient network for small target detection. The architecture exploits a small feature extractor based on Darknet20, as well as skip connection, via both bypass and concatenation, and reshape-passthrough layer to alleviate the vanishing gradient problem, promote feature reuse across network and combine low-level positional information with more meaningful high-level information. To verify the performances of YOLO-S, we build "AIRES", a novel dataset for cAr detectIon fRom hElicopter imageS acquired in Europe, and set up experiments on both AIRES and VEDAI datasets, benchmarking this architecture with four baseline detectors. Furthermore, in order to handle efficiently the issue of data insufficiency and domain gap when dealing with a transfer learning strategy, we introduce a transitional learning task over a combined dataset based on DOTAv2 and VEDAI and demonstrate that can enhance the overall accuracy with respect to more general features transferred from COCO data. YOLO-S is from 25% to 50% faster than YOLOv3 and only 15-25% slower than Tiny-YOLOv3, outperforming also YOLOv3 in terms of accuracy in a wide range of experiments. Further simulations performed on SARD dataset demonstrate also its applicability to different scenarios such as for search and rescue operations. Besides, YOLO-S has an 87% decrease of parameter size and almost one half FLOPs of YOLOv3, making practical the deployment for low-power industrial applications.

==> manuscript-bib.tex <==
\begin{thebibliography}{9}

\bibitem{Qu_2017} 
T. Qu, Q. Zhang and S. Sun, Vehicle detection from high-resolution aerial images using spatial pyramid pooling-based deep convolutional neural networks, Multimed. Tools Appl., Vol. 76, pp. 21651–21663, 2017.

\bibitem{Tang_2017} 
T. Tang, S. Zhou, Z. Deng, H. Zou, L. Lei, Vehicle Detection in Aerial Images Based on Region Convolutional Neural Networks and Hard Negative Example Mining, Sensors, Vol. 17, pp. 336, 2017

\bibitem{Ju_2019} 
M.~Ju, J.~Luo, P.~Zhang, M.~He and H.~Luo, A Simple and Efficient Network for Small Target Detection, IEEE Access, Vol. 7, pp. 85771-85781, 2019.

\bibitem{Razakarivony_2015} 
S.~Razakarivony, F.~Jurie, Vehicle Detection in Aerial Imagery: A small target detection benchmark, Journal of Visual Communication and Image Representation, Elsevier, 2015.

\bibitem{Xia_2018} 
G.~Xia, X.~Bay, J.~Ding, Z.~Zhu et al., DOTA: A Large-Scale Dataset for Object Detection in Aerial Images, IEEE/CVF Conference on Computer Vision and Pattern Recognition, pp. 3974-3983, 2018.

% Munich dataset
\bibitem{Liu_2015} 
K.~Liu, G.~Mattyus, Fast Multiclass Vehicle Detection on Aerial Images, IEEE Geosci. Remote Sens. Letters, Vol. 12, pp. 1938–1942, 2015.

% R-CNN
\bibitem{Girshick_2014} 
R.~Girshick, J.~Donahue, T.~Darrell, and J.~Malik, Rich feature 
hierarchies for accurate object detection and semantic segmentation, IEEE Conf. Comput. Vis. Pattern Recognit (CVPR), Columbus, OH, USA, pp. 580-587, 2014.

% Fast R-CNN
\bibitem{Girshick_2015} 
R.~Girshick, Fast R-CNN, IEEE Int. Conf. Comput. Vis. (ICCV), pp. 1440-1448, 2015.

\bibitem{Ren_2015} 
S. Ren, K. He, R. Girshick and J. Sun, “Faster R-CNN: Towards Real-Time Object Detection with Region Proposal Networks”, Proceedings of NIPS, 2015.

\bibitem{Redmon_2017} 
J.~Redmon and A.~Farhadi, YOLO9000: Better, faster, stronger, IEEE Conf. Comput. Vis. Pattern Recognit. (CVPR), pp. 6517-6525, 2017 

\bibitem{Redmon_2018} 
J.~Redmon and A.~Farhadi, Yolov3: An incremental improvement, \url{https://arxiv.org/abs/1804.02767}, 2018.

\bibitem{Bochkovskiy_2020} 
A.~Bochkovskiy, C.-Y.~Wang, H.-Y.~Mark~Liao, \url{https://arxiv.org/abs/2004.10934}, 2020.

\bibitem{Liu_2016} 
W.~Liu, D.~Anguelov, D.~Erhan, C.~Szegedy, S.~Reed, C.-Y.~Fu, A.~C.~Berg, SSD: Single Shot MultiBox Detector, European Conference on Computer Vision (ECCV), Lecture Notes in Computer Science, Springer, Vol. 9905, pp. 21-37, 2016

\bibitem{YOLO} 
YOLO: Real-Time Object Detection, \url{https://pjreddie.com/}

\bibitem{He_2019}
W.~He, Z.~Huang, Z.~Wei, C.~Li and B.~Guo, TF-YOLO: An Improved Incremental Network for Real-Time Object Detection, Applied Sciences, Vol. 9, pp. 3225, 2019. 

\bibitem{Cheng_2014}
G.~Cheng, J.~Han, P.~Zhou and L.~Guo, Multi-class geospatial object detection and geographic image classification based on collection of part detectors, ISPRS Journal of Photogrammetry and Remote Sensing, Vol. 98, pp. 119-132, 2014.

\bibitem{Cheng_2016}
G.~Cheng, P.~Zhou, J.~Han, Learning rotation-invariant convolutional neural networks for object detection in VHR optical remote sensing images, IEEE Transactions on Geoscience and Remote Sensing, Vol. 54, pp. 7405-7415, 2016.

\bibitem{Everingham_2010}
M.~Everingham, L.V.~Gool, C.~Williams, J.~Winn, A.~Zisserman, The Pascal Visual Object Classes (VOC) challenge, International Journal of Computer Vision, Vol. 88, pp. 303-338, 2010. 

\bibitem{Cao_2020}
C.~Cao, J.~Wu, X.~Zeng, Z.~Feng, T.~Wang, X.~Yan, Z.~Wu, Q.~Wu, Z.~Huang, Research on Airplane and Ship Detection of Aerial Remote Sensing Images Based on Convolutional Neural Network, Sensors, Vol. 20, pp. 4696, 2020.

\bibitem{Yang_2020}
G. Yang, Z. Tang and J. Huang, Vehicle-specific retrieval based on aerial images, IOP Conference Series. Materials Science and Engineering, Vol. 806, pp. 012049, 2020.

\bibitem{Rezatofighi_2019}
H. Rezatofighi, N. Tsoi, J. Gwak, A. Sadeghian, I. Reid and S. Savarese, Generalized Intersection Over Union: A Metric and a Loss for Bounding Box Regression, IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR), pp. 658-666, 2019.

\bibitem{Zhong_2017}
J.~Zhong, T.~Lei, G.~Yao, Robust Vehicle Detection in Aerial Images Based on Cascaded Convolutional Neural Networks, Sensors, Vol. 17, pp. 2720, 2017. 

\bibitem{Simonyan_2014}
K. Simonyan, A. Zisserman, Very Deep Convolutional Networks for Large-Scale Image Recognition, \url{https://arXiv 1409.1556}, 2014. 

\bibitem{Everingham_2015}
M. Everingham, S.M.A. Eslami, L. Van Gool, C.K.I. Williams, J. Winn, A. Zisserman, The Pascal Visual Object Classes Challenge: A Retrospective, Int. J. Comput. Vis., Vol. 111, pp. 98–136, 2015.

%\bibitem{COCO_challenge}
%COCO Detection Challenge (Bounding Box). Available online: \url{https://competitions.codalab.org/%competitions/20794}

\bibitem{Lin_2014} T.-Y.~Lin, M.~Maire, S.~Belongie, J.~Hays et al, Microsoft COCO: Common Objects in Context”, Computer Vision - ECCV 2014, Lecture Notes In Computer Science (Springer), Vol. 8693, pp. 740-755, 2014.

\bibitem{Deng_2009}
J. Deng, W. Dong, R. Socher, L. -J. Li, Kai Li and Li Fei-Fei, ImageNet: A large-scale hierarchical image database, IEEE Conference on Computer Vision and Pattern Recognition, pp. 248-255, 2009.

\bibitem{LabelImg} \url{https://github.com/tzutalin/labelImg}

\bibitem{Lin_2016}
T.Y.~Lin, P.~Dollar, R.~Girshick, K.~He et al, Feature pyramid networks for object detection, IEEE Conference on Computer Vision and Pattern Recognition, Honolulu, HI, pp. 936-944, 2016.

\bibitem{Yosinski_2014}
J. Yosinski, J. Clune, Y. Bengio and H. Lipson, How transferable are
features in deep neural networks?, Proceedings of the 27th International Conference on Neural Information Processing Systems, Vol. 2, pp. 3320-3328, 2014.

\bibitem{Alganci_2020}
U. Alganci, M. Soydas, E. Sertel, Comparative Research on Deep Learning Approaches for Airplane Detection from Very High-Resolution Satellite Images, Remote Sensing, Vol. 12, pp. 458, 2020.

\bibitem{Padilla_2021}
R.~Padilla, W.L.~Passos, T.L.B.~Dias, S.L.~Netto and E.A.B.~da~Silva, A Comparative Analysis of Object Detection Metrics with a Companion Open-Source Toolkit, Electronics, Vol. 10, pp. 279, 2021. 

\bibitem{Vestias_2019}
M. P. Véstias, A Survey of Convolutional Neural Networks on Edge with Reconfigurable Computing, Algorithms, Vol. 12, pp. 154, 2019.

\end{thebibliography}


